Self-supervised Video Transformer

In this paper, we propose self-supervised training for video transformers using unlabeled video data. From a given video, we create local and global spatiotemporal views with varying spatial sizes and frame rates. Our self-supervised objective seeks to match the features of these different views representing the same video, to be invariant to spatiotemporal variations in actions. To the best of our knowledge, the proposed approach is the first to alleviate the dependency on negative samples or dedicated memory banks in Self-supervised Video Transformer (SVT). Further, owing to the flexibility of Transformer models, SVT supports slow-fast video processing within a single architecture using dynamically adjusted positional encoding and supports long-term relationship modeling along spatiotemporal dimensions. Our approach performs well on four action recognition benchmarks (Kinetics-400, UCF-101, HMDB-51, and SSv2) and converges faster with small batch sizes. Code: https://git.io/J1juJ

==> figures/ablation_aug.tex <==
\begin{table}[t]
	\centering
	\begin{tabular}{c|c|c}
		\toprule
		Method          & UCF     & HMDB  \\  \midrule
		w/o standard aug & 84.20   & 52.10 \\
		standard aug     & \textbf{84.64}   & \textbf{52.17} \\ \bottomrule
	\end{tabular}
    \caption{\textbf{Ablation Study for Standard Augmentations.} Using standard spatial augmentations including Colour Jitter, Random Grayscaling, Gaussian Blur, and Solarization leads to some performance improvement. }
    \label{tbl:ablation_aug}
\end{table}


==> figures/ablation_fr.tex <==
\begin{table}[t]
	\centering
	\begin{tabular}{c|c|c|c}
		\toprule
		TV     &  CVC         & UCF     & HMDB  \\  \midrule
		\xmark &  \xmark      & 73.81   & 42.91 \\
		\cmark &  \xmark $^*$ & 82.41   & 44.55 \\ 
		\xmark &  \cmark      & 83.58   & 50.66 \\ 
		\cmark &  \cmark      & \textbf{84.64}   & \textbf{52.17} \\ \bottomrule
	\end{tabular}
    \caption{\textbf{Ablation Study for Temporal Views.} We study the performance gains with our proposed temporal views (TV) separately and when applied with cross-view correspondences (CVC). Note that TV without CVC still involves multiple views of a single video ($^*$). }
    \label{tbl:ablation_temporal_aug}
\end{table}


==> figures/ablation_inference.tex <==
\begin{table}[t]
	\centering
	\begin{tabular}{c|c|c}
		\toprule
		Method          & UCF     & HMDB  \\  \midrule
		single-view     & 84.64   & 52.17 \\
		multi-view      & \textbf{84.80}   & \textbf{53.15} \\ \bottomrule
	\end{tabular}
    \caption{\textbf{Ablation Study for Slow-Fast Inference.} Our slow-fast inference strategy that makes use of dynamic positional embedding boosts the performance on downstream tasks.}
    \label{tbl:ablation_inf}
\end{table}


==> figures/ablation_tc.tex <==
\begin{table}[t]
	\centering
	\scalebox{1}{
	\begin{tabular}{c|c|c|c|c|c}
		\toprule 
		L$\to$G  & G$\to$G  & L$\to$L  & G$\to$L & UCF     & HMDB  \\  \midrule
		\cmark   & \xmark   & \xmark   & \xmark  & 84.11   & 50.72 \\ 
		\xmark   & \cmark   & \xmark   & \xmark  & 81.95   & 49.04 \\ 
		\cmark   & \cmark   & \xmark   & \xmark  & \textbf{84.64}   & \textbf{52.17} \\
		\cmark   & \cmark   & \cmark   & \xmark  & 83.11   & 51.23 \\
		\cmark   & \cmark   & \xmark   & \cmark  & 84.71   & 51.88 \\
		\cmark   & \cmark   & \cmark   & \cmark  & 83.69   & 51.71 \\ \bottomrule
	\end{tabular}
	}
    \caption{\textbf{Ablation study on temporal correspondences.} We further study the various types of temporal correspondences presented in \cref{subsec:cross_view_corrspondences}. Jointly predicting local to global and global to global correspondences along temporal dimension results in optimal performance for downstream tasks. Note that X$\to$Y is predicting Y from X, where X,Y take values L, G local and global respectively.}
    \label{tbl:ablation_correspondences}
\end{table}


==> figures/baseline.tex <==
\begin{table}[t]
	\centering\small
	\setlength{\tabcolsep}{7pt}
	\scalebox{1.0}[1.0]{
	\begin{tabular}{c|c|c|c}
		\toprule
		\rowcolor{Gray} 
		Spatial  & Temporal & UCF-101     & HMDB-51 \\ \midrule
		\cmark   & \xmark   & 73.81   & 42.91   \\ 
		\xmark   & \cmark   & 82.90   & 42.59   \\ 
		\cmark   & \cmark   & \textbf{84.64}   & \textbf{52.17}   \\ \bottomrule
	\end{tabular}}
    \caption{\textbf{Ablation study on cross-view correspondences.} We study the effect of each component of our proposed correspondences. The baseline case involves only spatial correspondences between views of videos. While temporal correspondences alone also obtains improvements, the joint application of both spatial and temporal correspondences learns representations optimal for both downstream tasks.}
    \label{tbl:baseline}
\end{table}



==> sections/experiments_old.tex <==
\section{Experiments}

\label{sec:experiments}

\input{figures/sota_k400}
\input{figures/sota_comp}
\input{figures/sota_ssv2}

\input{figures/baseline}
\input{figures/ablation_tc}
\input{figures/ablation_fr}
\input{figures/ablation_inference}
\input{figures/ablation_aug}

\subsection{Experimental Setup and Protocols}

\textbf{Architecure}: We build over the ViT architecture and training framework from \cite{gberta_2021_ICML, fan2020pyslowfast, rw2019timm, caron2021emerging}. 

\textbf{Datasets:} 
Kinetics-400 \cite{kinetics400} is a large-scale dataset containing 240k training videos and 20K validation videos belonging to 400 different action classes. On average, these videos are of duration around 10 seconds, with 25 frames per second (i.e., around 250 frames per video). UCF-101 \cite{soomro2012ucf} and HMBD-51 \cite{kuehne2011hmdb} are two small-scale datasets each containing 13K videos belonging to 101 classes and 5K videos belonging to 51 classes respectively. Something-Something v2 (SSv2) \cite{goyal2017something} is another large-scale dataset heavily focused on motion with 168k training and 24k validation videos belonging to 174 action classes. Unlike UCF101 and HMDB51 which contain action classes similar to Kinetics-400, SSv2 contains very different actions involving complex human object interactions, such as “Moving something up” or “Pushing something from left to right”. 

%In addition to our proposed approaches for view generation, we use standard data augmentations (random flips and colour jitter) on our inputs similar to recent work \cite{qian2020spatiotemporal}. and  

\textbf{Training:} We train our models for 100 epochs on the train set of Kinetics-400 dataset \cite{kinetics400} using a batch size of 32 across 4 NVIDIA-A100 GPUs. This batch size refers to the number of unique videos present within a given batch. However, the effective input batch size to network would be higher because of our view generation process (multiple global and local temporal views of a same video \cref{subsec:cross_view_corrspondences}). We randomly initialize weights relevant to temporal attention while spatial attention weights are initialized using a ViT model trained in a self-supervised manner over the ImageNet-1K dataset \cite{imagenet}.  We used an Adam optimizer \cite{kingma15adam} with a learning rate of $5e-4$ scaled using a cosine schedule with linear warmup for 5 epochs \cite{Steiner2021HowTT, chen2021mocov3}. We also use weight decay scaled from 0.04 to 0.1 during training. 

\textbf{Evaluation:} We evaluate the transferability of our self-supervised representations for action recognition on UCF-101 \cite{soomro2012ucf}, HMDB-51 \cite{kuehne2011hmdb}, and SSv2 \cite{goyal2017something} datasets. Additionally, similar to recent work, we also evaluate on the Kinetics-400 \cite{kinetics400} dataset.
For each dataset, we perform two evaluations, 1) training a linear classifier over our pre-trained ViT backbone, 2) fine-tuning our pre-trained network with linear classifier end-to-end.

\textbf{Linear Evaluation:} We train a linear classifier over our pretrained ViT backbone (which is frozen during training) for 100 epochs with a batch size of 32 on a single NVIDIA-V100 GPU. We use SGD with an initial learning rate of 1e-3 with a cosine decay schedule and momentum of 0.9. Our networks for downstream tasks are trained on the train splits and evaluated on the validation splits (split 1 for UCF / HMDB) of each dataset. For each video, we extract 8 equally sampled frames of size 224. For evaluation, in line with previous work, we extract 3 different spatial crops of the each video sampling 8 frames per crop.   

\textbf{Finetuning:} The pre-trained network is used for initialization and the model is trained end-to-end for 15 epochs with a batch size of 32 across 4 NVIDIA-V100 GPUs. Following the supervised training methodology for space-time ViTs on videos \cite{gberta_2021_ICML}, we use SGD with a learning rate of 5e-3 decayed by a factor of 10 at epochs 11 and 14, momentum of 0.9, and weight decay of 1e-4.  

\subsection{Comparison to state-of-the-art}
\textbf{Kinetics-400:}
We first compare our approach against recent state-of-the-art on Kinetics-400 dataset \cite{kinetics400}. Our results are presented in \cref{tbl:sota_k400}. Our approach obtains state-of-the-art performance on the Kinetics validation set for both linear evaluation and fine-tuning settings. Unlike recent work that uniformly samples 10 clips from the full-length videos with 3 crops each, we use a single clip of 8 frames covering the entire video and use 3 crops for that clip. 

\textbf{UCF-101 \& HMDB-51:}
Taking advantage of our dynamic positional encoding, we deploy Slow-Fast inference for these datasets. We next compare our method against recent work on UCF-101 \cite{soomro2012ucf} and HMDB-51 \cite{kuehne2011hmdb} datasets. We present these results in \cref{tbl:sota_comp}. Our methods out-performs state-of-the-art for UCF-101 and is on-par for HMDB-51.
In these evaluations, we sample two clips per video at different spatio-temporal resolutions, (8x224x224) and (16x96x96), and obtain 3 spatial crops for each clip.  

\textbf{SSv2:}
We also compare our methods on SSv2 \cite{goyal2017something} datasets obtaining state-of-the-art performance. We highlight how this is a more difficult dataset requiring in-depth motion understanding to learn the complex human object interactions that differentiate classes.   Given how multiple SSv2 classes share similar background and object appearance with complex movements being the key differentiating factors \cite{Hu_2021_ICCV}, these results illustrate how our representations capture strong motion related contextual information. 

\subsection{Ablative Analysis}
We conduct ablative studies on each component of our proposed approach to verify their contribution to our overall performance gains. For these experiments, we use a subset of the Kinetics-400 train set containing 60,000 videos for the self-supervised training. Evaluation is carried out over an alternate split of UCF and HMDB datasets. We train our models for 20 epochs using the same setup detailed above and evaluate similarly as well.

% We conduct ablative studies on each component of our proposed approach to verify their contribution to our overall performance gains. For these experiments, we use a subset of the Kinetics-400 train set containing 60,000 videos for the self-supervised training. Evaluation is carried out over an alternate split of UCF and HMDB datasets. We train our models for 20 epochs using the same setup detailed above and evaluate similarly as well (\cref{subsec:exp_setup}). Across these experiments, we maintain a constant computational complexity by adjusting batch sizes as necessary to compensate for additional / larger views introduced. 

\textbf{Cross-View Correspondences.} Since self-supervised training requires some form of view generation method, a simple baseline for comparison is setup using only spatial correspondences for the self-supervised training. This involves predicting spatially local and global views of videos from each other. We replace this with our proposed temporal correspondences and also joint temporal and spatial correspondences. Results detailed in \cref{tbl:ablation_correspondences} shows how correspondences across both dimensions leads to optimal performance. We further study all possible cross-view correspondences along the temporal dimension involving various predictions between local and global views. These results are presented in ~\cref{tbl:ablation_correspondences}. Predicting global views from local and alternate global views results in optimal performance on downstream tasks.  

% The optimal combination of local to global and global to global correspondences in \cref{tbl:ablation_correspondences} involves view generation by jointly limiting the field of view along both spatial and temporal dimensions. We explore the effect of limiting the field of view across each dimension separately in \cref{tbl:ablation_st}. Note how separately limiting the view is optimal for each dataset along a different dimension (temporal for UCF-101 and spatial for HMDB-51), indicating the different kinds of correspondences learned through each constraint. Moreover, our proposed approach of jointly limiting views across both dimensions leads to optimal performance for both datasets.

\textbf{Motion Prediction.} We also evaluate our proposed temporal views which involves varying of video sampling rates. We present these results in \cref{tbl:ablation_temporal_aug}. Jointly enforcing motion prediction and cross-view correspondences results in optimal performance. We note that predicting local views from global or alternate local views did not lead to performance improvements. In these experiments, the batch sizes are varied to maintain constant compute usage since varying correspondences leads to additional views per video (and hence larger effective batch sizes). 

\textbf{Slow-Fast Inference.} We evaluate our proposed inference strategy in \cref{tbl:ablation_inf}. We note the higher gains in HMDB-51 \cite{kuehne2011hmdb} where the classes are easier to separate with motion information \cite{han2020self}. 

\textbf{Augmentations}: We also explore the impact standard augmentations have on our method in \cref{tbl:ablation_aug}. While we obtain insignificant gains on HMDB-51, we are able to obtain some gain over UCF-101 dataset.  

% We study the impact of standard augmentations \cite{qian2020spatiotemporal} on our method in \cref{tbl:ablation_aug}. Using these augmentations results in superior performance; although we obtain insignificant gains on HMDB-51, we are able to obtain visible gains over UCF-101 dataset.

==> sections/introduction_old.tex <==
\section{Introduction}
\label{sec:intro}

Self-supervised learning promises to extract meaningful representations from the unlabeled data, alleviating the need for expensive annotations. Recent self-supervised methods perform on-par with supervised learning for certain vision tasks \cite{he2020momentum, chen2020simple, caron2018DeepCF, caron2020unsupervised}. In domains such as video analysis where annotations are more expensive, self-supervised learning is all the more promising which can exploit the presence of temporal information for learning better feature representations \cite{recasens2021broaden, Jenni_2021_ICCV, Huang_2021_ICCV}. 

At the same time, the emergence of vision transformers (ViTs) \cite{dosovitskiy2020image} and their successful adoption to different computer vision tasks including video understanding \cite{gberta_2021_ICML, liu2021video, Ryoo2021TokenLearnerWC, sharir2021image, arnab2021vivit, fan2021multiscale} within the supervised setting show their promise in the video domain. In fact, recent works using simple ViT backbones \cite{gberta_2021_ICML} surpass convolutional neural network (CNN) baselines for the supervised video analysis with reduced compute. 
%Further, self-supervision has also been shown to learn meaningful features beyond their supervised counterparts under various settings \cite{caron2021emerging}. 
Motivated by the ability of self-attention to model long range dependencies, we propose a simple yet effective method to train video transformer \cite{gberta_2021_ICML} in a self-supervised manner that can use temporal information as a supervisory signal from the unlabelled video data to learn motion, scale and viewpoint invariant features. 

\input{figures/intro}

Existing self-supervised video representation learning works \cite{xie2016unsupervised, recasens2021broaden, qian2020spatiotemporal}  use contrastive learning objectives which require larger batch sizes, longer training regimes, careful negative mining and/or dedicated memory banks. Further, the contrastive objectives require careful temporal sampling \cite{qian2020spatiotemporal} and multiple networks looking at similar/different clips to develop attract/repel loss formulations \cite{recasens2021broaden}. In contrast, we propose to learn self-supervised features from unlabelled video data via self-distillation \cite{tarvainen2017mean} by twin network strategy (student and teacher) \cite{grill2020bootstrap, caron2021emerging}.  The student and teacher have exactly the same network architecture which is based on TimeSformer \cite{gberta_2021_ICML} and our approach trains these models with a similarity objective \cite{caron2021emerging} that matches the representations along spatial and temporal dimensions by space and time attention \cite{gberta_2021_ICML}. We achieve this by creating spatiotemporal positive views that are sampled at different time frames from a same video but also differs in spatial size (Fig.~\ref{fig:architecture}). During training, teacher video transformer parameters are updated as an exponential moving average of the student video transformer (Fig.~\ref{fig:architecture}). Both of these networks process different spatiotemporal views of the same video (Sec. \ref{subsec:cross_view_corrspondences}) and our loss then predicts one video clip from the other in the feature space. This way our approach learns robust features that are invariant to spatiotemporal changes in  a video while generating discriminative features across videos \cite{grill2020bootstrap}. Therefore, our method does not depend on negative mining or large batch sizes and remains computationally efficient as our approach converges within few epochs ( $\approx$ 20 on Kinetics-400 \cite{kinetics400}). 

\noindent Real-world actions can occur with varying motion and spatial details, however, current self-supervised methods based video frameworks operate on fixed spatial and temporal scales which can can pose difficulties in modeling the expressivity and dynamic nature of actions. 3D Convolutional Networks have been commonly used as a backbone for video processing networks \cite{xiao2021modist, qian2020spatiotemporal}. However, they lack the adaptability to varying temporal resolutions (due to fixed number of channels) and thus require dedicated networks for each temporal resolution \cite{feichtenhofer2019slowfast, kahatapitiya2021coarse}. 
% \knr{This is in contrast to the image domain where a single network is trained to handle images of varying spatial resolution.}
Our approach on the other hand is designed to benefit from varying spatial and temporal details within the same network.  We use a video transformer \cite{gberta_2021_ICML} based approach that can handle varying temporal resolutions within the same architecture using dynamically adjusted positional encodings (Sec. \ref{subsec:dynamic_positional_embedding}). Furthermore, the self-attention mechanism in video transformers  can capture both local and global long-range dependencies across both space and time, offering much larger receptive fields as compared to traditional convolutional kernels \cite{naseer2021intriguing}. 

We introduce novel mechanism for self-supervised training of video transformers by exploiting motion as a supervisory signal only from RGB data modality. Our contributions are:

\begin{enumerate}[leftmargin=*,noitemsep]
	\item \emph{\textbf{Motion as Prediction:}} We propose novel training mechanism to extract meaningful supervisory signals by modeling motion characteristics from unlabelled videos. Our approach only uses RGB data modality and the success of our self-supervised features across various datasets highlights that motion prediction can alleviate the need for expensive video annotation (Sec. \ref{sec:experiments}).    
	\item \emph{\textbf{Novel Spatiotemporal Sampling:}}  In order to use motion as prediction task, we propose novel sampling strategies to create target labels. Specifically, we generate global and local sptiotemporal views with vary frame rates and spatial characteristics (Fig. \ref{fig:architecture} and Sec. \ref{subsec:cross_view_corrspondences}). These views are then matched by our global to global and local to global prediction function using self-distillation from a teacher and student models \cite{caron2021emerging} (Sec. \ref{subsec:svt_loss}). 
	\item \emph{\textbf{Dynamic Positional Encodings:}} We propose to use dynamic positional encoding within a single video transformer \cite{gberta_2021_ICML} to handle variable frame rate results from our sampling strategy (Sec. \ref{subsec:dynamic_positional_embedding}).
\end{enumerate}

Our extensive experiments and results on various video dataset including Kintics-400, UFC-101, HMDB-51, and SSv2 show state-of-the-art transfer of our self-supervised features. Further, our method shows rapid convergence rate.


% The unique characteristic of video inputs is the presence of temporal and spatial dimensions. Given the high redundancy of information in videos, it is common to sample a video at a much lower temporal resolution (frame-rate) than its original in video analysis tasks for improving computational complexity. However, higher resolution in each dimension can provide finer detail. Sampling each dimension separately at varying resolutions to extract multiple sets of finer features has been successful in CNNs using separate backbones for each resolution \cite{feichtenhofer2019slowfast, kahatapitiya2021coarse}.

% In the case of self-supervised learning, contrastive methods have emerged most successful recently \cite{he2020momentum, caron2020unsupervised}. While this initially involved negative samples, recent works focus on predicting alternate views (augmented or differently sampled versions) of a sample \cite{caron2021emerging, recasens2021broaden}. In particular, predicting global information from local patches has been successful in both image \cite{caron2020unsupervised, caron2021emerging} and video \cite{recasens2021broaden} domains. 

% In this work, we propose a novel self-supervised methodology for learning video representations using ViT backbones. To the best of our knowledge, this is a first work that explores the behaviour of video ViTs under self-supervised learning settings. We also explore video sampling at varying resolution with ViT architectures, video view generation by limiting locality for predictive self-supervision, and sharing a common network backbone for different resolution inputs.

% Most existing self-supervised video representation learning works \cite{han2020self, xiao2021modist, qian2020spatiotemporal, Hu_2021_ICCV} use contrastive learning objectives requiring larger batch sizes, longer training regimes, customized negative mining strategies, dedicated memory banks, and / or alternate input modalities. Recent works using predictive losses \cite{recasens2021broaden} use separate networks for different views. In contrast, our approach relies on alternate view prediction as the self-supervised objective sharing a common backbone for distinct views. This leads to more computational efficiency and faster convergence while dropping the need for negative mining, memory banks, large batch sizes, and multiple network architectures. Further, inspired from \cite{caron2021emerging, he2020momentum}, we use a teacher-student setup where our teacher model is an exponential moving average (EMA) of the student. While our teacher model consumes alternate views to generate targets for the predictive objective, only the student model requires training due to the EMA setup, unlike methods using two separate network backbones. 

% Multiple recent video self-supervised learning works also explore the idea of varying resolution along temporal dimension \cite{Huang_2021_ICCV, chen2021rspnet}. They use contrastive losses between different videos at same resolution for speed consistency or the same video at different resolutions for appearance consistency. In our work, we jointly vary spatio-temporal resolution and use a different predictive objective as self-supervision.  

% The idea of views with limited locality is explored in \cite{Behrmann2021LongSV, recasens2021broaden}. While \cite{Behrmann2021LongSV} uses views of varying locality for disentangling the representation space into temporally local and global features using contrastive objectives, our approach uses view locality to learn correspondences along and across dimensions with our predictive objective. A similar predictive objective with temporal locality constrained views is used in \cite{recasens2021broaden}; however our approach focuses on spatio-temporal constraints extending correspondences across dimensions, uses a single shared network for processing alternate views, and additionally combines varying resolutions to generate our alternate views. 

% Finally, in contrast to recent self-supervised video representation works, our approach uses a ViT backbone in our architecture. We incorporate dynamic positional embedding during training to handle our multiple views of varying resolution within a single shared backbone. Our method also allows using multiple different resolution views during inference for improved performance on tasks with rapid temporal movement or longer videos.  



% % \noindent 
% In summary, our contributions are as follows:
% \begin{enumerate}[topsep=1pt,itemsep=-0.5ex,partopsep=0ex,parsep=1ex]
% 	\item We present an end-to-end vision transformer based approach for self-supervised video representation learning (a first to the best of our knowledge)
% 	\item Obtain fast self-supervised training convergence with a predictive objective between different views using a single shared network (EMA teacher and student)
% 	\item Propose novel view generation approach involving video sampling at variable spatio-temporal resolution and limited locality
% \end{enumerate}



==> sections/method_old.tex <==
\section{Self-supervised Video Transformers}
\label{sec:method}

% \subsection{Motivation} 
% Existing self-supervised video representation learning works \cite{xie2016unsupervised, recasens2021broaden, qian2020spatiotemporal}  use contrastive learning objectives which require larger batch sizes, longer training regimes, careful negative mining and/or dedicated memory banks. Further, the contrastive objectives require careful temporal sampling \cite{qian2020spatiotemporal} and multiple networks looking at similar/different clips to develop attract/repel loss formulations \cite{recasens2021broaden}. In contrast, we propose to learn self-supervised features from unlabelled video data via self-distillation \cite{tarvainen2017mean} by twin network strategy (student and teacher) \cite{grill2020bootstrap, caron2021emerging}.  The student and teacher have exactly the same network architecture which is based on TimeSformer \cite{gberta_2021_ICML} and our approach trains these models with a similarity objective \cite{caron2021emerging} that matches the representations along spatial and temporal dimensions by spatiotemporal attention \cite{gberta_2021_ICML}. We achieve this by creating spatiotemporal positive views that are sampled at different time frames from a same video but also differs in spatial size (Fig.~\ref{fig:architecture}). During training, teacher video transformer parameters are updated as an exponential moving average of the student video transformer (Fig.~\ref{fig:architecture}). Both of these networks process different spatiotemporal views of the same video (Sec. \ref{subsec:cross_view_corrspondences}) and our loss then predicts one video clip from the other in the feature space. This way our approach learns robust features that are invariant to spatiotemporal changes in  a video while generating discriminative features across videos \cite{grill2020bootstrap}. Therefore, our method does not depend on negative mining or large batch sizes and remains computationally efficient as our approach converges within few epochs ( $\approx$ 20 on Kinetics-400 \cite{kinetics400}). 

% \noindent Real-world actions can occur with varying motion and spatial details, however, current self-supervised methods based video frameworks operate on fixed spatial and temporal scales which can can pose difficulties in modeling the expressivity and dynamic nature of actions. 3D Convolutional Networks have been commonly used as a backbone for video processing networks \cite{xiao2021modist, qian2020spatiotemporal}. However, they lack the adaptability to varying temporal resolutions (due to fixed number of channels) and thus require dedicated networks for each temporal resolution \cite{feichtenhofer2019slowfast, kahatapitiya2021coarse}. 
% % \knr{This is in contrast to the image domain where a single network is trained to handle images of varying spatial resolution.}
% Our approach on the other hand is designed to benefit from varying spatial and temporal details within the same network.  We use a video transformer \cite{gberta_2021_ICML} based approach that can handle varying temporal resolutions within the same architecture using dynamically adjusted positional encodings (Sec. \ref{subsec:dynamic_positional_embedding}). Furthermore, the self-attention mechanism in video transformers  can capture both local and global long-range dependencies across both space and time, offering much larger receptive fields as compared to traditional convolutional kernels \cite{naseer2021intriguing}. 

% (a) Existing self-supervised video representation learning works use contrastive learning objectives which require larger batch sizes, longer training regimes, careful negative mining and/or dedicated memory banks. Further, the contrastive objectives require multiple networks looking at similar/different sub-sequences to develop attract-repel loss formulation. 

% (b) Existing SSL based video frameworks consider fixed spatial and temporal scales during learning. Since real-world actions can occur with varying speeds and spatial details, operation on a single scale can pose difficulties in modeling the expressivity and dynamic nature of actions. 

% (c) 3D Convolutional Networks have been commonly used as a backbone for video processing networks . However, they lack the adaptability to varying temporal resolutions (due to fixed number of channels) and thus require dedicated networks for each temporal resolution. In contrast, our ViT based approach can handle varying temporal resolutions within the same architecture using dynamically adjusted positional encodings. Furthermore, the self-attention mechanism in ViTs can capture both local and global long-range dependencies across both space and time, offering much larger receptive fields as compared to traditional convolutional kernels. 


\subsection{Proposed Approach: SVT} 
% \knr{ As illustrated in \cref{fig:architecture}, SVT learns by predicting alternate views of varying locality and resolution, i.e. predicting global views with higher locality and resolution from local views of lower locality and resolution. 
%By varying locality, we refer to sampling by cropping along spatial and temporal dimensions of a video.} \muz{I think we are describing these details down in the text. Perhaps we can remove this text.}

In contrast to contrastive constraints, we process two clips from the same video with varying spatial and temporal details (Sec.~\ref{subsec:dynamic_positional_embedding}) which avoids the need for any negative mining or memory bank. Our loss formulation matches the representations from both dissimilar clips to enforce invariance to motion and spatial changes for the same action. This approach simultaneously incorporates rich spatio-temporal context while keeping them discriminative \cite{grill2020bootstrap}. 

Our self-supervised training framework is based on reconstructing multi-scale and multi-rate (i.e., varying spatial and temporal resolutions) feature representations across frames, thereby encouraging the model to learn contextual cues across space and time. In terms of different scales, our two branches (Fig.~\ref{fig:architecture}) operate on local vs. global views and seek to reconstruct one from the other. Instead of using a fixed frame rate, we use different frame rates in the student and teacher networks to account for speed variations in actions and modeling long-term temporal context in videos using attention. To this end, we use ViT with separate attention for the temporal and spatial dimensions of inputs similar to \cite{gberta_2021_ICML}.


\subsection{SVT: Architecture}

We apply separate attention along temporal and spatial dimension of the video clips using vision transformer \cite{gberta_2021_ICML}. Our ViT comprises of 12 encoder blocks and can process video clips of size $(B\times  C\times T\times W\times H)$, where $B$ and $C$ represent the batch size and number of color channels, respectively, while the maximum spatial and temporal sizes are $W=H=224$ and $T=16$, respectively. In other words, we only sample 16 frames from a given video and rescale these frames to $224\times 224$. Our network architecture (Fig.~\ref{fig:architecture}) is designed to process variable input resolution during training such as varying frame rate, number of frames in a video clip (Sec. \ref{subsec:cross_view_corrspondences}) and difference in spatial size. However, each ViT encoder block processes at maximum of 196 spatial and 16 temporal tokens and embedding dimension of each token is $\mathbb{R}^{m}$ \cite{dosovitskiy2020image}. In addition to these input spatial and temporal tokens, we also use a single classification token as the feature vector within the architecture \cite{devlin2018bert}. This classification token represents the common features learned by the ViT along spatial and temporal dimension of a given video. Note that we use variable spatial and temporal resolutions that is  $W \le 224$, $H \le 224$ and $T \le 16$. The variations in the input resolution results in a variable number of spatial and temporal tokens during training. We use the single class token to accommodate varying spatial and temporal token counts along with the dynamic positional encoding (Sec. \ref{subsec:dynamic_positional_embedding}). Finally, we use a projection head over the class token from the final ViT encoder \cite{caron2021emerging, grill2020bootstrap}. 

\textbf{Self-Distillation.} As illustrated in \cref{fig:architecture}, our overall approach uses a teacher-student setup inspired from \cite{caron2021emerging, grill2020bootstrap} for self-distillation \cite{tarvainen2017mean}. Our teacher model is an exact architectural replica of the student model (including the ViT backbone and the predictor MLP). The teacher model does not undergo any direct training. During each training step of the student model, we update the teacher weights as an exponential moving average (EMA) of the student weights \cite{caron2021emerging}. This allows us to use a single shared network for processing multiple input clips. 


\subsection{SVT: Training}
Given the high temporal dimensionality of videos, motion and spatial characteristics of an action such as walking or playing tennis changes during the video. Thus a number of distinct video clips with different motion characteristics can be sampled from a single video. A key novelty of our approach involves predicting these different video clips with varying temporal characteristics from each other in the feature space. This leads to learning contextual information defining the underlying distribution of videos and makes the network invariant to motion, scale and viewpoint variations. Thus,  we formulate self-supervision for video representation learning as a motion prediction problem which has three key components: \textbf{a)} We generate multiple temporal views consisting of different numbers of clips with varying motion characteristics from the same video (Sec. \ref{subsec:mo_pred} ), \textbf{b)} In addition to motion, we vary spatial characteristics of these views as well by generating local (smaller spatial field) and global (higher spatial field) of the sampled clips (Sec. \ref{subsec:cross_view_corrspondences}), and \textbf{c)} We introduce a loss function that matches the varying views across spatial and temporal dimensions in the latent space.


\subsubsection{Motion Prediction as Self-supervision}
\label{subsec:mo_pred}
A defining characteristic of a video is the frame rate (number of frames sampled from a video) and varying the frame rate can change the motion context of a video (e.g. walking slow vs walking fast) while controlling nuanced actions (e.g. subtle body-movements of walking action). 
In general, video clips are sampled at a fixed frame rate \cite{qian2020spatiotemporal, xiao2021modist}. However, given two views of varying frame rate (different number of total clips for each view), predicting one from the other in feature space explicitly involves modelling the motion of objects across those clips. Further, predicting subtle movements captured at high frame rates will force a model to learn motion related contextual information from a low frame rate input. 

\textbf{Temporal Views:} We refer to a collection of clips sampled at a certain frame rate from a given video as a temporal view. We generate different views by sampling at different frame-rates which produces temporal views with varying resolution. This means that number of temporal tokens ($T$) input to ViT vary in different views. Our proposed method enforces the correspondences between such views which allows to capture different motion characteristics of the same action. We create random sampling of these views to create motion differences among them. These views are processed by our ViT models and we predict one view from the other in the latent space. In addition to varying temporal resolution, we also vary the resolution of clips across the spatial dimension within these views. This means that spatial size of a clip can be lower than the maximum spatial size (224) which can also decrease the number of spatial tokens.   Similar sampling strategies have been used \cite{feichtenhofer2019slowfast, kahatapitiya2021coarse} but under multi-network settings while our approach handles such variability in temporal resolutions with a single ViT model by using dynamic positional encoding (Sec. \ref{subsec:dynamic_positional_embedding}). %Moreover, for a given view, lower spatial resolutions allows increasing temporal resolution significantly while maintaining a fixed compute requirement. 

%Using lower spatial resolutions for certain views allows increasing their temporal resolution significantly while maintaining a fixed compute requirement
% We randomly sample two views of the same video at different frame rates, project them to the feature space of our model, and predict each feature from the other. This can be compared to commonly used random resizing of images which introduces priors regarding spatial consistency to the model. At the same time,
% we note how this operation involves no interpolation but simply sampling at varying rates resulting in the presence of distinct information in certain views.




\subsubsection{Cross-View Correspondences}
\label{subsec:cross_view_corrspondences}
Our training strategy aims at learning the relationships across both temporal and spatial dimensions from a given video. To this end, we propose novel cross-view correspondences by altering the field of view during sampling. To achieve this, we generate global and local temporal views from a given video. \textbf{Global Temporal Views:} We randomly sample $T=8$ or $T=16$ clips from a video with spatial size fixed to $W=H=224$. We always generate two global temporal views. \textbf{Local Temporal Views:} Local views cover a limited portion of the video both along spatial and temporal dimensions. We generate local temporal views by randomly sampling number of clips $T\in\{2,4,8,16\}$ with spatial size fixed to $W=H=96$. We always generate eight local temporal views during training.  \textbf{Augmentations:} We apply different data augmentations to spatial dimension that is to the clips sampled for each view. Specifically, we apply color jittering and gray scaling with probability 0.8 and 0.2, respectively to all the temporal views. We further apply gaussian blur and solarization with probability 0.1 and 0.2, respectively to global temporal views.

Our intuition is that predicting a global temporal view of a video from a local temporal view in the latent space forces the model to learn high-level contextual information by modeling \textbf{a)} spatial context in the form of possible surrounding of a given spatial crop, and \textbf{b)} temporal context in the form of possible previous or future clips from a given temporal crop. Note that the spatial correspondences also involve a temporal component that is for a given clip from local view at time stamp $t=i$, our approach also tries to predict a global view at time stamp $t=j$. These cross-view correspondences are enforced by our similarity objective (Eq. \ref{eq:svt_loss}) that predict different views from each other. 

%the presence of contextual information across time in a spatially local view. These correspondences are enforced by predicting different views (local and global) from each other. We next discuss our approach for obtaining different views of a video in detail. 

\textbf{Routing between ViTs:} Cross-view correspondences consists of the local and global temporal views that are different from each other both spatially and temporally. We adapt a simple routing strategy that randomly selects and forwards these views through the networks \eg student ViT can see either of the local or global view during training at a certain epoch. Our proposed cross-view correspondences combined with the routing mechanism allows to model motion characteristics by predicting global views from the local views and also predicting one global view from the other.  Therefore, our proposed approach enforces learning the contextual information across all dimensions of a video. 



%Our method exploits predicting of cross-view correspondences under four settings along with their various combinations. We define a global view as a crop containing a fraction of the video (along either spatial or temporal dimensions) higher than a selected threshold. A local view is a similar fraction lower than a (different) selected threshold. Therein, for a given video, we explore the effects of predicting a global view from,
% \begin{itemize}[topsep=3pt,itemsep=-1ex,partopsep=0ex,parsep=1ex]
% 	\item spatially local crops 
% 	\item spatially alternate global views 
% 	\item temporally local crops
% 	\item temporally alternate global views 
% \end{itemize}
% While we also explore additional correspondences predicting local views from global views, the ones listed above result in optimal performance.   

% These correspondences we learn span across both spatial and temporal dimensions allowing representations to learn better contextual awareness along each dimension. 

% In particular, the combined application of these approaches (e.g. predicting a spatially-global temporally local view from a spatially-local temporally global view)  specifically requires learning contextual information across all dimensions of a video. 

% In detail, all views we generate (both local and global across both dimensions) are random crops of videos either along the spatial dimensions or the temporal dimension. In the case of spatial crops, local views correspond to a random crop covering a smaller spatial region (below a selected area threshold) of a video while a global crop refers to a random crop covering a large spatial region (above a selected area threshold). The same applies for temporal crops, where a randomly selected crop (set of consecutive frames) spans below or above selected time thresholds for local and global views respectively. 

% These views are generated jointly with varying temporal resolution to enforce motion prediction as well. We note that the resolution of each view is another factor that will vary, which we discuss next. 


\subsubsection{Dynamic Positional Embedding}
\label{subsec:dynamic_positional_embedding}

Vision transformers \cite{dosovitskiy2020image} process sequences of tokens in parallel and use positional encoding to model sequence ordering \cite{naseer2021intriguing}. Interestingly, positional encoding also allows ViT to process variable input sizes by interpolating the positional embeddings for the missing tokens. We use this property of positional encoding to our advantage to accommodate varying spatial and temporal resolution of our proposed temporal views during training. We alter the number of input spatial and temporal tokens during training with limited modifications to the model architecture or weights. However, the positional embedding which injects positional information to each token needs to be altered during training. We use a separate postional embedding vector for spatial and temporal dimension and fix our positional embedding vectors to the highest resolution across each dimensions. We vary these vectors through interpolation during training to account for the missing spatial or temporal tokens. This allows our single ViT model to process inputs of varying resolution while also giving the positional embedding a dynamic nature which are more suited for different sized inputs in the downstream tasks.   

% We note how ViTs allow easy manipulation of input resolution by varying the number of tokens which is widely used in image related tasks \cite{pmlr-v139-touvron21a, caron2021emerging}. These methods use a fixed-length positional embedding during training followed by interpolation of embedding for different length inputs during fine-tuning or inference. 

% Given the common characteristic in space-time ViT architectures \cite{gberta_2021_ICML} of using separate temporal attention to make all tokens temporally aware followed by self-attention with a class token over the spatial dimension, we are able to alter the number of input tokens during training with limited modifications to the model architecture or weights. Varying input tokens in turn allows inputs of varying resolution across dimensions. However, the positional embedding which injects positional information to each token needs to be altered during training. We fix our positional embedding vector to the highest resolution across each dimensions and vary it through interpolation during training. This allows our single network to consume inputs of varying resolution while also giving the positional embedding a dynamic nature (more suited for different sized inputs in downstream tasks).   

\subsection{SVT Loss}
\label{subsec:svt_loss}
SVT is trained with the objective function (Eq. \ref{eq:svt_loss}) that predicts different views from each other. These views represent different spatial variations that are sampled at different time stamps and belong to a same video.  Our approach considers these views as positive pairs that are shifted along the temporal dimension and SVT objective function (Eq. \ref{eq:svt_loss}) matches these views sampled at different time stamps to find motion invariant feature representations. 

Consider a given a video $\bm{X}=\{\bx_t\}_{t=1}^N$, where $N$ represent number of 
% clips/ : people refer to a subvideo as clip in literature
frames. Let $\bm{V}_{g}$ and $\bm{V}_{l}$ represent global and local temporal views such that $\bm{V}_{g}=\{\bx_t\}_{t=1}^{K_{g}}$ and $\bm{V}_{l}=\{\bx_t\}_{t=1}^{K_{l}}$, where $\bm{V}_{g}$ and $\bm{V}_{l}$ are subsets of video $\bm{X}$ and $K_{l} \le K_{g}$. We randomly sample two global and eight local temporal views (Sec. \ref{subsec:cross_view_corrspondences}). These temporal views are passed though the student and teacher models to get the corresponding class tokens or features $\bm{f}_g$ and $\bm{f}_l$. These class tokens are normalized as follows: 

\begin{equation}
     \bm{\Tilde{f}}^{(i)} = \frac{\text{exp}(\bm{f}^{(i)}) / \tau}{\sum_{n=1}^m \text{exp}(\bm{f}^{(i)})/ \tau },
\end{equation}

where $\tau$ is a temperature parameter used to control sharpness of exponential function \cite{caron2021emerging}.  


% $\tau_{a} (X_{i}), \tau_{b} (X_{i})$ be two views of the video generated inline with our proposed method.  Let $H_{s/t}, G_{s/t}$ be the backbone ViT and predictor networks respectively for student / teacher networks. We define $f_{i,j, k} = H_k (\tau_{j}(X_i) )$ such that $f_{i, a, s}, f_{i, b, t}$ are two views (from $\tau_{a}$ and $\tau_{b}$) of video $X_{i}$ in representation space of the student ($s$) and teacher ($t$) network respectively. We define the normalized feature vector $\hat f_{i,j,k}$ as, 
% \begin{equation}
%     \hat f_{i,j,k}[p] = \frac{exp(f_{i,j,k}[p]) / t_k}{\sum_{n=1}^N exp(f_{i,j,k}[n] / t_k)}
% \end{equation}
% which involves a softmax computed over the feature dimension (of size N). Here $f[p]$ refers to the $p^\text{th}$ value of vector $f$ and $t_k$ is a temperature parameter used to control sharpness of exponential function.  

\textbf{Global to Global Spatiotemporal Loss:} Our two global temporal views have same spatial size but differs in temporal content as number of clips/frames are randomly sampled for each view. One of the global temporal view is always passed through the teacher model which serve as the target label. We map the global temporal view of the student with the teacher to create global to global temporal loss.

\begin{align}\label{eq:global_to_global_loss}
    \mathcal{L}_{gg} &=  -\bm{\Tilde{f}}_{g_{t}} * log(\bm{\Tilde{f}}_{g_{s}}),
\end{align}
where, $\bm{\Tilde{f}_{g_{s}}}$ and $\bm{\Tilde{f}_{g_{t}}}$ are the class tokens for global temporal views produced by the student and teacher, respectively.


% Using these normalized features, our base loss function is cross-entropy loss computed as follows, which we minimize w.r.t. to the parameters $\theta_s$ of our joint student network $H_s$ and  $G_s$:
% \begin{align}
%     \mathcal{L}_\text{base}(a, b) &= \sum_{i} - \hat f_{i,b,t} * log(\hat f_{i,a,s})
% \end{align}
% where the summation is over a mini-batch and the output of the teacher network (weights frozen), $\hat f_{i, b, t}$, is considered the fixed target. 


\textbf{Local to Global Temporal Loss:} Our local temporal views have limited field of vision both along spatial and temporal dimensions when compared with the global temporal view. However, the number of local views are 4 times higher than global views. All the local temporal views are passed through the student model and mapped to global temporal view from the teacher model.

\begin{align}\label{eq:local_to_global_loss}
    \mathcal{L}_{lg} &= \sum_{n=1}^{q} -\bm{\Tilde{f}}_{g_{t}} * log(\bm{\Tilde{f}}^{(n)}_{l_{s}}),
\end{align}

Where $q$ represents the number of local temporal views which is set to eight in all of our experiments. The overall loss to train SVT is simply a linear combination of both losses (Eq. \ref{eq:global_to_global_loss}, and \ref{eq:local_to_global_loss} ) and given as follows:

\begin{equation}\label{eq:svt_loss}
    \mathcal{L} =  \mathcal{L}_{lg} +  \mathcal{L}_{gg}
\end{equation}


% The overall loss involves a set of functions used to obtain various views of a single video. We define $\tau_{l}$ and $\tau_{g}$ to randomly sample local and global views respectively (as described in \cref{subsec:cross_view_corrspondences} \& \cref{subsec:dynamic_positional_embedding}). Our overall loss can then be presented as follows:

% \begin{equation}\label{eq:svt_loss}
%     \mathcal{L} = \mathcal{L}_\text{base}(l, g) + \mathcal{L}_\text{base}(g, g)
% \end{equation}



\subsection{SVT: Inference}
Increasing the input resolution of videos across either dimension (spatial / temporal) can benefit inference due to the presence of additional videos. Using two different views, a) high spatial low temporal resolution b) low spatial high temporal resolution, during inference allows to capture finer-information across both dimensions with minimal increase in computation. This is common in recent work that use two-networks for processing videos at different resolutions \cite{feichtenhofer2019slowfast, kahatapitiya2021coarse}. 

In our case, given how we feed video inputs sampled at varying resolutions to our backbone during the self-supervised training phase, we extend the same to inference. Prior to inference on a downstream task, we attach an MLP (linear classifier in our experiments) over our backbone followed by fine-tuning either only the MLP or the entire network. We feed multiple views (varying spatio-temporal resolution) of a video to the backbone to extract multiple features per video. These features are combined and then fed to the MLP for obtaining final predictions. 

In comparison to inputs at a single resolution, our approach allows extracting finer details from videos across each dimension. We also reiterate how our approach uses a single common backbone for each resolution.
